Non-Parametric Stochastic Sequential Assignment With Random Arrival Times

We consider a problem wherein jobs arrive at random times and assume random values. Upon each job arrival, the decision-maker must decide immediately whether or not to accept the job and gain the value on offer as a reward, with the constraint that they may only accept at most $n$ jobs over some reference time period. The decision-maker only has access to $M$ independent realisations of the job arrival process. We propose an algorithm, Non-Parametric Sequential Allocation (NPSA), for solving this problem. Moreover, we prove that the expected reward returned by the NPSA algorithm converges in probability to optimality as $M$ grows large. We demonstrate the effectiveness of the algorithm empirically on synthetic data and on public fraud-detection datasets, from where the motivation for this work is derived.

==> spare_text.tex <==

% \begin{theorem}
% Let $X$ be a random variable with support on $[0, U]$ and associated mean shortage function $\phi$.
% Then, the estimate of the mean shortage function returned by Algorithm~\ref{alg:ecdf_mean_shortage} converges in probability to the true value, that is,
% $$\lim_{N \to \infty} \mathbb{P} \qty[ \max_{y \in [0, U]} \abs{\widetilde{\phi}_{\text{E}}^{(N)}(y) - \phi(y)} > \epsilon] = 0$$
% for any $\epsilon > 0$, where the estimate computed by Algorithm~\ref{alg:ecdf_mean_shortage} using $N$ independent samples of $X$ is denoted by $\widetilde{\phi}_{\text{E}}^{(N)}(y)$.
% \end{theorem}
% \begin{proof} % y \in [0, U]
% Denote the cdf of $X$ by $F$ and the empirical cdf computed from $N$ independent samples of $X$ by $F_N(x)$.
% It follows from the specification of Algorithm~\ref{alg:ecdf_mean_shortage} that $\widetilde{\phi}_{\text{E}}^{(N)}(y) = \int^U_y (1 - F_N(x)) \dd x$ as the integral of a piecewise constant function is the sum of the areas of the corresponding rectangles and $F_N$ is a piecewise constant function with domain $[0, U]$.

% Now suppose that $\sup_{x \in [0, U]} \abs{F(x) - F_N(x)} < \gamma$ for some $\gamma > 0$. Then, for any $y \in [0, U]$,

% \noindent\resizebox{\columnwidth}{!}{
%   \begin{minipage}{\linewidth}
%   \begin{align}
%     \abs{\widetilde{\phi}_{\text{E}}^{(N)}(y) - \phi(y)} &= \abs{ \textstyle\int^U_y (1 - F(x)) \dd x - \textstyle\int^U_y (1 - F_N(x)) \dd x } \nonumber \\
%     &= \abs{ \textstyle\int^U_y (F_N(x) - F(x)) \dd x } \nonumber \\
%     &\leq \textstyle\int^U_y \abs{F_N(x) - F(x)} \dd x \nonumber \\
%     &\leq \textstyle\int^U_y \gamma \dd x = \gamma(U - y) \leq \gamma U.  \label{eq:ecdf_consistency_ineq}
% \end{align}
%   \end{minipage}
% }
% Fix an arbitrary $\epsilon > 0$ and suppose that $\abs*{\widetilde{\phi}_{\text{E}}^{(N)}(y) - \phi(y)} > \epsilon$.
% Moreover, introduce a variable parameter $\delta > 0$.
% Either $\abs{F(y) - F_N(y)} \geq \delta$ or $y \in B_\delta$, where we define $B_\delta := \left\{x \in [0, U] \middle\vert \abs{F(x) - F_N(x)} < \delta,\ \abs*{\widetilde{\phi}_{\text{E}}^{(N)}(x) - \phi(x)} > \epsilon \right\}$.
% Extending to many realisations of the $N$ samples of $X$,
% \begin{multline}\label{eq:ecdf_consistency_prob_sum}
%     \mathbb{P}\left[\abs*{\widetilde{\phi}_{\text{E}}^{(N)}(y) - \phi(y)} > \epsilon \right] \leq \mathbb{P}\left[\abs{F(y) - F_N(y)} \geq \delta \right] \\+ \mathbb{P}\left[y \in B_\delta \right].
% \end{multline}
% Setting $\delta \leq \epsilon / U$ gives us $B_\delta = \emptyset$ from Equation~\eqref{eq:ecdf_consistency_ineq} and so $\mathbb{P}\left[y \in B_\delta \right] = 0$.
% Substituting into Equation~\eqref{eq:ecdf_consistency_prob_sum} yields
% \begin{equation*}
%     \mathbb{P}\left[\abs*{\widetilde{\phi}_{\text{E}}^{(N)}(y) - \phi(y)} > \epsilon \right] \leq \mathbb{P}\left[\abs{F(y) - F_N(y)} \geq \frac{\epsilon}{U} \right].
% \end{equation*}
% Now let $y' = \arg\max_{y\in[0, U]} \abs*{\widetilde{\phi}_{\text{E}}^{(N)}(y) - \phi(y)}$.
% Since we have allowed $y \in [0, U]$ to be arbitrary
% \begin{multline}
%     \label{eq:ecdf_consistency_preDKW}
%     \mathbb{P}\left[ \abs*{\widetilde{\phi}_{\text{E}}^{(N)}(y') - \phi(y')} > \epsilon \right] \leq \mathbb{P}\left[\abs{F(y') - F_N(y')} \geq \frac{\epsilon}{U} \right] \\ 
%     \leq \mathbb{P}\left[\sup_{z \in [0, U]} \abs{F(z) - F_N(z)} \geq \frac{\epsilon}{U} \right],
% \end{multline}
% where the second inequality follows from the fact that $\abs{F(x) - F_N(x)} \geq \xi \Rightarrow \sup_{z \in [0, U]} \abs{F(z) - F_N(z)} \geq \xi$ for all $x \in [0, U]$, $\xi > 0$.
% Employing the Dvoretzky–Kiefer–Wolfowitz inequality~\cite{dvoretzky1956,massart1990} for the rightmost term in~\eqref{eq:ecdf_consistency_preDKW},
% \begin{equation*}
%     \mathbb{P}\left[\abs*{\widetilde{\phi}_{\text{E}}^{(N)}(y') - \phi(y')} > \epsilon \right] \leq 2\exp(-\frac{2N\epsilon^2}{U^2}).
% \end{equation*}
% Finally, passing to the limit as $N \to \infty$ gives the result.
% \end{proof}




% \subsection{Adjusted value distribution via Kernel Density Estimation (KDE)}

% \begin{lemma}
% Suppose $X \sim \operatorname{LogNormal}(\mu, \sigma)$ and define
% $$\phi(y) := \int^\infty_y (x - y) f_X(x) \dd x,$$ 
% where $f_X$ is the pdf of $X$. Then,

% \begin{multline}
%     \phi(y) = \frac{1}{2} e^{\mu + \frac{\sigma^2}{2}} \left( 1 + \erf\left( \frac{\mu + \sigma^2 - \ln(y)}{\sigma \sqrt{2}} \right) \right) \\ 
%     - \frac{y}{2} \left( 1 + \erf\left( \frac{\mu - \ln(y)}{\sigma \sqrt{2}} \right) \right) , 
% \end{multline}
% where $\erf(z) = \frac{2}{\sqrt{\pi}} \int^z_0 e^{-t^2} \dd t$. 
% \end{lemma}
% \begin{proof}
%     \todo[inline]{prove it}
% \end{proof}

